Efficient Stepping Algorithms and Implementations for Parallel Shortest Paths

In this paper, we study the single-source shortest-path (SSSP) problem with positive edge weights, which is a notoriously hard problem in the parallel context. In practice, the $\Delta$-stepping algorithm proposed by Meyer and Sanders has been widely adopted. However, $\Delta$-stepping has no known worst-case bounds for general graphs. The performance of $\Delta$-stepping also highly relies on the parameter $\Delta$. There have also been lots of algorithms with theoretical bounds, such as Radius-stepping, but they either have no implementations available or are much slower than $\Delta$-stepping in practice. We propose a stepping algorithm framework that generalizes existing algorithms such as $\Delta$-stepping and Radius-stepping. The framework allows for similar analysis and implementations of all stepping algorithms. We also propose a new ADT, lazy-batched priority queue (LaB-PQ), that abstracts the semantics of the priority queue needed by the stepping algorithms. We provide two data structures for LaB-PQ, focusing on theoretical and practical efficiency, respectively. Based on the new framework and LaB-PQ, we show two new stepping algorithms, $\rho$-stepping and $\Delta^*$-stepping, that are simple, with non-trivial worst-case bounds, and fast in practice. The stepping algorithm framework also provides almost identical implementations for three algorithms: Bellman-Ford, $\Delta^*$-stepping, and $\rho$-stepping. We compare our code with four state-of-the-art implementations. On five social and web graphs, $\rho$-stepping is 1.3--2.5x faster than all the existing implementations. On two road graphs, our $\Delta^*$-stepping is at least 14\% faster than existing implementations, while $\rho$-stepping is also competitive. The almost identical implementations for stepping algorithms also allow for in-depth analyses and comparisons among the stepping algorithms in practice.

==> algo-framework.tex <==
%\begin{algorithm}[t]
%\caption{The Stepping Algorithm Framework.\label{alg:framework}}
%\SetKwFor{parForEach}{ParallelForEach}{do}{endfor}
%\KwIn{A graph $G=(V,E,w)$ and a source node $s$.}
%\KwOut{The graph distances $d(\cdot)$ from $s$.}
%    \vspace{0.5em}
%%$S_0\leftarrow \{s\}$\\
%\DontPrintSemicolon
%$\delta[\cdot]\leftarrow +\infty$, associate $\delta$ to $Q\in \PQ$\\
%$\delta[s]\leftarrow 0$, $Q.\lazyinsert{}(s)$\\
%\While{$|Q|>0$\label{line:while-loop}} {
%\parForEach {$u\in Q.\extract(\extcond)$\label{line:extract}} {
%    \parForEach{$v\in N(u)$\label{line:innerloop2}} {
%    \If {$\WriteMin(\delta[v],\delta[u]+w(u,v))$ succeeds \label{line:writemin}} {
%      $Q.\lazyinsert{}(v)$
%    }
%  }
%}
%Execute \finishcond\tcp*[f]{\small \normalfont for \deltas and \radiuss}
%}
%\Return {$\delta(\cdot)$}\\[.25em]
%\end{algorithm}


\begin{table*}
{\centering
(\textbf{This is Figure Page 3.} This page gives the \BDPQ{} interface and stepping algorithm framework. )
\vspace{0.2in}
}\\
\begin{minipage}{1.5\columnwidth}
  \def\arraystretch{1.25}
  {\centering
  \begin{tabular}{@{}p{2.5cm}@{  }@{  }p{5.5cm}@{}}
    \hline
    % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
    %$Q=$\build{}$()$:& $\seq\langle I\times K \times V\rangle\mapsto \PQ$ & Initialize the \BDPQ{} from a sequence of id-key-value \record{} \\
    %\multicolumn{2}{l}{\bf Plain \BDPQ:}\\
    $Q.\lazyinsert(\id)$: \flushright$\PQ \times I \mapsto \Box$ & Modify the \record{} with identifier $\id$ in $Q$. If $\id\notin Q$, add it to $Q$ with current $\delta[\id]$. If $\id\in Q$, notify $Q$ that $\delta[\id]$ has changed and needs to update before the next \extract.\\
    $s=Q.$\extract{}$(\theta)$:\flushright $\PQ\times K\mapsto \seq$& Return identifiers in $Q$ with keys no more than $\theta$ and delete them from $Q$.\\
%    \hline
%    \multicolumn{2}{l}{\bf With augmentation:}\\
%    $a=Q.\collect()$:\flushright $\PQ\mapsto A$& Compute the abstract sum of all elements in $Q$ defined by a binary operator $\oplus$ \\
    \hline
  \end{tabular}
  \caption{\textbf{Interface of \BDPQ{}.} \label{tab:interface}}
  }
\end{minipage}
%\hspace{.5em}

\begin{minipage}{1.2\columnwidth}
{%
\begingroup
\removelatexerror% Nullify \@latex@error
\begin{algorithm*}[H]
\caption{The Stepping Algorithm Framework.\label{alg:framework}}
\SetKwFor{parForEach}{ParallelForEach}{do}{endfor}
\KwIn{A graph $G=(V,E,w)$ and a source node $s$.}
\KwOut{The graph distances $d(\cdot)$ from $s$.}
    \vspace{0.5em}
%$S_0\leftarrow \{s\}$\\
\DontPrintSemicolon
$\delta[\cdot]\leftarrow +\infty$, associate $\delta$ to $Q\in \PQ$\\
$\delta[s]\leftarrow 0$, $Q.\lazyinsert{}(s)$\\
\While{$|Q|>0$\label{line:while-loop}} {
\parForEach {$u\in Q.\extract(\extcond)$\label{line:extract}} {
    \parForEach{$v\in N(u)$\label{line:innerloop2}} {
    \If {$\WriteMin(\delta[v],\delta[u]+w(u,v))$ succeeds \label{line:writemin}} {
      $Q.\lazyinsert{}(v)$
    }
  }
}
Execute \finishcond\tcp*[f]{\small  for \deltas and \radiuss}
}
\Return {$\delta(\cdot)$}\\[.25em]
\end{algorithm*}
\endgroup}
\end{minipage}

\vspace{5em}
\input{table-framework}

\vspace{5in}
\end{table*}


==> algo-tour-tree.tex <==
%%\begin{minipage}{\columnwidth}
%\begin{algorithm}%[H]
%%\small
%\caption{The Tournament-tree based \BDPQ.\label{alg:tour-tree}}
%
%%\SetKwFor{parForEach}{ParallelForEach}{do}{endfor}
%\SetKw{KwMaintain}{Maintains}
%\KwMaintain{A \tourt $T$ with $n$ leaf nodes each corresponds to a record.}
%    \vspace{0.5em}
%%$S_0\leftarrow \{s\}$\\
%\DontPrintSemicolon
%\SetKwBlock{InPar}{In Parallel:}{}
%\SetKwProg{myfunc}{Function}{}{}
%
%\myfunc{\upshape \addmark(record id $\id$, flag $\mb{newflag}$)} {
%  Let $t$ be the tree leaf corresponding to \mb{id}\\
%  $t.\inQ\gets \mb{newflag}$\\
%  \While {\upshape $t\ne T.root$ and $\TAS(t.\wtparent.\updated)$} {
%    $t\gets t.\wtparent$
%  }
%}
%\codeskip{}
%\myfunc{\upshape \wtupdate(node $t$) $\to k\in K$\label{line:update-start}} {
%  \If {$t$ is leaf} {
%    \lIf{$t.\mb{inQ}$} {\Return{$\delta[t.id].k$}}
%    \lElse {\Return{$+\infty$}
%  }
%  }
%  \lIf {$t.\updated=0$} {\Return{$t.k$}\tcp*[f]{no further update}}
%  $t.\updated \gets 0$\\
%  \InPar {
%    $\mb{leftKey}\gets \wtupdate(t.\wtleft)$\\
%    $\mb{rightKey}\gets \wtupdate(t.\wtright)$
%  }
%  \Return {$t.k \gets\min(\mb{leftKey}, \mb{rightKey}$)}\label{line:update-end}
%}
%\codeskip{}
%\myfunc{\upshape \traverse(threshold $\theta$, node $t$) $\to \mb{seq}$\label{line:traverse-start}} {
%  \If {$t$ is a leaf} {
%    \addmark($t.\id, 0$)\label{line:delete} \tcp*{Marked as not in Q}
%    \Return{$\{t.\mb{id}\}$}
%  }
%  \lIf {$\theta<t.k$} {\Return{$\{\}$}\tcp*[f]{empty seq}}
%  \InPar {
%    $\mb{leftseq}\gets\traverse(\theta,t.\wtleft)$\\
%    $\mb{rightseq}\gets\traverse(\theta,t.\wtright)$
%  }
%  \Return $\mb{leftseq}+\mb{rightseq}$\label{line:traverse-end}
%}
%\codeskip{}
%\myfunc{\upshape \extract(threshold $\theta$)} {
%  $\wtupdate(T.\mb{root})$\\
%  \Return $\traverse(\theta,T.\mb{root})$
%}
%\codeskip{}
%\myfunc{\upshape \lazyinsert($\id$)} {
%  $\addmark(\id{},1)$\\
%}
%\end{algorithm}



\begin{figure*}
(\textbf{This is Figure Page 4.} This page illustrates the \tourt{} data structure for \BDPQ{}, and also contains a table summarizing the bounds for the stepping algorithms. )\\
    %\begin{subfigure}{.5\textwidth}
    %    \myalgorithm
    %    \caption{How to write algorithms}
    %\end{subfigure}% need this comment symbol to avoid overfull hbox
%    \begin{minipage}{1.1\columnwidth}
%      \myalgorithm
%    \end{minipage}
%    \begin{minipage}{0.9\columnwidth}
%      \includegraphics[width=\columnwidth]{figures/tour-tree-illu.pdf}
%  \caption{\textbf{An illustration for a tournament tree.}  Square leaf nodes store the records and each round internal node keeps the smallest key in the corresponding subtree. (a) is simply an illustration of the \tourt{} containing 6 records $3,8,4,6,1$ and $5$. (b) shows an update on a batch of $3,8$ and $6$. The shaded nodes will be marked as \emph{modified}.\label{fig:tour-tree}}
%    \end{minipage}
%    \begin{subfigure}{.5\textwidth}
%        %\myalgorithm
%        \caption{How to write algorithms}
%    \end{subfigure}
%\caption{Main caption}
%\vspace{2em}
\input{table-bounds}
\vspace{5in}
\end{figure*}


==> app-tourtree-proof.tex <==
\section{Full Details and Analysis of Theoretically Efficient \BDPQ}\label{sec:app-tour-tree-cost}



We now give the proof of \cref{thm:main-tour-tree}.
We first analyze the functions in \cref{alg:tour-tree}.

\begin{lemma}
\label{lem:wtfunctions}
Consider a \tourt{} on a universe of $n$ records, implemented with algorithms in \cref{alg:tour-tree}.
Given $b$ invocations of \addmark{} function in a batch, the total cost of these \addmark{} functions is $O\left(b\log\frac{n}{b}\right)$.
If there are $b$ invocations of \addmark{} function in the last batch, the total cost of the \wtupdate{} is $O\left(b\log\frac{n}{b}\right)$.
If the \traverse{} algorithm extracts $b$ (smallest) elements from \tourt{} $T$, the total cost of \traverse{} is $O\left(b\log\frac{n}{b}\right)$.
\end{lemma}
\begin{proof}
  We first show that, in a \tourt{}, for a subset $X$ of tree leaves, if we denote $S(X)$ as the set of all ancestors of nodes in $X$, then $|S(X)|=O\left(|X|\log\frac{n}{|X|}\right)$.
  This has been shown on more general self-balanced binary trees \cite{Blelloch2016justjoin,blelloch2018geometry}, and just a simplified case suffices as \tourt{s} are complete binary trees.

  First, \addmark{} modifies the flag $\updated$ for each tree path node all modified leaves to the root. Let $X$ be all tree leaves corresponding to the invocations \addmark{} functions in this batch. Therefore $|X|=b$.
  By definition of $S(X)$, we know that only nodes in $X\cup S(X)$ are visited.
  Because of the \tas{} operation, a node $v\in S(X)$ recursively call \addmark{} on its parent $u$ if and only if $v$ successfully set the $\updated$ mark of $u$. This means that for any interior node $u\in S(X)$, this can happen only once. Therefore, every node in $S(X)$ is visited by the \addmark{} function at most once. This proves that the cost of all \addmark{} functions $O\left(b\log\frac{n}{b}\right)$.

  For \wtupdate{}, it restores all relevant interior tree nodes top-down. Let $X$ be all tree leaves corresponding to the invocations \addmark{} functions in the last batch (so that they need to be addressed in this \wtupdate{}). Therefore $|X|=b$.
  Note that the algorithm skips a subtree when the $\updated$ flag is \false{}. Therefore, the total number of visited nodes must be a subset of all nodes in $X\cup S(X)$ and their children. Given that each node has at most two children, this number can also be asymptotically bounded by $|X\cup S(X)|$, which are those marked \true{} in the $\updated$ flags. This gives the same bound as the total cost of \addmark{} functions in a batch.

  For \extract{}, denote the leaves corresponding to all the output \record{s} as set $X$ of size $b$.
  Note that we skip a subtree if its key (minimum key in its subtree) is larger than $\theta$. This means that we visit an interior node only if at least one of its descendants will be included in the output batch. Therefore, all visited nodes are also $X\cup S(X)$ and all their children.
  For all visited leaves, \extract{} also calls \addmark{} to set $\mb{inQ}$ flag to 0 (\false). As proved above, the total cost of these \addmark{} functions is $O\left(b\log\frac{n}{b}\right)$.
  Therefore, the total cost of \traverse{} is also $O\left(b\log\frac{n}{b}\right)$ to extract a batch of size~$b$.
\end{proof}

With \cref{lem:wtfunctions} that shows the cost of each function in \cref{alg:tour-tree}, we can now formally prove \cref{thm:main-tour-tree}.

\medskip
\begin{proof}[Proof of \cref{thm:main-tour-tree}]
  Recall that the \emp{modification work} on a batch $B$ as all work paid to \lazyinsert{} all \record{s} in $B$, as well as any later work (possibly done by a later \extract{}) to actually apply the updates, and the \emp{extraction work} on a batch $B$ is all work paid to output the batch from the \extract{} function, as well as any later work (possibly done by the next \extract{}) to actually remove them from $Q$. In \tourt{}, the modification work includes all \addmark{} operations called by the \lazyinsert{} functions in the batch, as well as later cost in the \wtupdate{} operation to restore keys of all the relevant interior nodes. From \cref{lem:wtfunctions}, the total cost is $O(b\log(\frac{n}{b}))$ for a batch of size $B$.
  The extraction work on a batch $B$ includes the work done by \traverse{} to get the output sequence, as well as to restore keys of all the relevant interior nodes in the next \wtupdate{}.

  For both \extract{} and \lazyinsert{}, the span is no more than the height of the tree, which is $O(\log n)$.
\end{proof}

%We note that the augmentation can also be maintained on winning tree easily. In particular, we will maintain the augmented value of each subtree at the subtree root. Because the binary operation $\oplus$ is communicative and associative, we compute the augmented value of a tree node by combining the augmented values of its two children. This can be maintained along the way of the \wtupdate{} algorithm. Reading the augmented value of the entire tree only requires $O(1)$ time because it is stored at the root.


==> conn-old.tex <==
\section{Parallel Soft Priority Queue}
\label{sec:sssp}
Another typical example of abstract data type (ADT) is the priority queue (\pq{}).
A priority queue maintains a set of elements with keys as priorities, and supports three primitives: \mf{Extract-Min} that pops the element with the smallest key, \mf{Insert} that adds a new element, and \mf{Dec-Key} that decreases the key of an element.
Other operations such as \mf{Delete} or \mf{Update} can be implemented via these primitives.
Priority queues have many applications, such as in Prim's algorithm~\cite{prim1957shortest} in computing minimum spanning tree, constructing Huffman tree~\cite{huffman1952method}, and best-first searches~\cite{pearl1984intelligent}.
The most famous application of priority queues is probably in Dijkstra's algorithm that efficiently computes the single-source shortest path (\sssp{}) on a graph.
Sequentially, Dijkstra's algorithm is simple and practical.
Similar to the previous section, we will use SSSP and Dijkstra as a motivating example for parallel priority queues.

As oppose to many graph algorithms, SSSP is notoriously hard in the parallel setting.
To date, there is no work-efficient (or even close to) solution with non-trivial ($o(n)$) span bound.
Directly parallelizing Dijkstra's leads to $\Omega(n)$ span due to the use of priority queue: \mf{Extract-Min} pops one vertex at a time for $n$ times in total.
There are two major attempts to parallelize the priority queue.
One is to allow concurrent updates to the priority queue \cite{}.
Hence, processors can work on different vertices together in Dijkstra, but the \mf{Extract-Min}s from the priority queue are still sequentialized.
The other attempt is to relax the priority queue to allow batch updates and batch extracts on $k$ elements, so multiple processors can work on different vertices simultaneously.
To support these functions, the underlying data structure is a search tree, which can be either the parallel search trees by the PI and coauthors~\cite{Blelloch2016just,sun2018pam,sun2019parallel} in the shared-memory setting or B-trees \cite{} in the distributed setting.
Unfortunately, maintaining the search tree is very costly because the total ordering of all elements are kept, which is not required in the sequential heap implementations.

One could also use the parallel BST \cite{} proposed by one of the PIs as a batched priority queue (as is used in \cite{}). However, maintaining an extra tree structure is less I/O-friendly in practice.
Interestingly, the work-inefficient Bellman-Ford algorithm is easier to be parallelized: in each round, all vertices attempt to relax all their neighbors, which can be done fully in parallel. Previous work has shown that this algorithm is easy to implement and have reasonable performance in many cases \cite{}.
Although Bellman-Ford is far from work-efficient and is almost trivial to parallelize, to the date, there is no parallel \sssp{} algorithm that is more efficient than Bellman-Ford both in theory (better worst-case bounds) and practice (better performance).

Due to the problems in aforementioned parallel priority queues, both theoretical and practical parallel SSSP algorithms \emph{do not} use the priority queue abstraction.
In practice, Bellman-Ford can easily be parallelized.
In each \step{}, only a subset of vertices are used to relax their neighbors, noted as the \emph{frontier}.
The algorithm maintains a queue buffering all vertices that recently have their distance updated, but have not yet relaxed their neighbors.
The frontier is extracted from the queue by a predefined condition (noted as $\condex$), which usually selects vertices close to the source. After that, relaxed vertices will update their priority and be added to the queue.
In other words, these algorithms already use a conceptual \emph{\bpq{}}, although not explicitly.
For example, the \deltastepping~\cite{meyer2003delta} algorithm uses all vertices with tentative distance $\le i\times \Delta$ in the frontier for \step{} $i$, where $\Delta$ is a graph-specific parameter. Due to its simplicity, \deltastepping{} is the most widely-used parallel \sssp{} algorithm in practice, and is adopted in many graph processing systems \cite{dhulipala2017julienne,hang2020optimizing,nguyen2013lightweight,BeamerAP15}. \deltastepping{} does not have worst-case time bound because the parameter $\Delta$ highly depends on the input graph structure and edge weight, and its best choice is not known before running the algorithm itself.
On the theory side, the state-of-the-art parallel \sssp{} theoretical result is the \radiusstepping{} algorithm, which was proposed by the PIs.
Instead of pushing out the frontier by a fixed distance as in \deltastepping{}, \radiusstepping{} changes the parameter $\Delta$ dynamically, noted as the current \emph{radius} $r_i$. The radius is decided based on the current frontier. Using this idea, \radiusstepping{} achieves worst-case work and span bounds and good parallelism (work-span ratio). There also exists other theory work using similar idea such as Shi and Spencers \cite{}. However, these algorithms are not used in practice because they require a preprocessing phase to add shortcuts. In practice, this could bring up serious space and time overhead.

We summarize the framework of frontier-based \sssp{} algorithm in Algorithm \ref{algo:sssp}.
All these high-level idea of these algorithms for \sssp{} shows similarity of employing a ``batched \pq{}'' conceptually (the \fname{SoftPQ}) structure in Algorithm \ref{algo:sssp}).
Namely, the condition function $\condex$ defines the priority, and the frontier is selected based on this priority.
Instead of one element, $\frontiersymbol$ is extracted as batch.
$\condex$ can be defined not only based on the value of a single key, but also more complex criteria. As such, we call this abstract data type a \emph{Soft Batched Priority Queue} (\emph{\sbpq{}}).
Surprisingly, however, none of the previous work formally studies this abstraction and semantics of the parallel \pq{} for the \sssp{} problem.
This is probably due to the use of this batched \pq{} is not as straightforward: instead of extracting a batch and process it in every round (noted as \step{s}) and repeat, there are also some ``\substep{s}'' (Line \ref{line:substep}). When processing the current frontier, a relaxed vertex may be ``pulled'' into the frontier and will be processed in the same \step{}, if some condition (noted as $\condadd$) is satisfied. Usually this condition checks if the tentative distance is smaller enough. This allows the frontier to grow dynamically, and aims at reducing both work and span of the algorithm. First, the vertices with small tentative distance should be used to relax other vertices as early as possible to avoid redundant relaxation. Secondly, processing more vertices in the same round reduces the number of \step{s}, and allows more work to do in parallel in the same \step{}, which improves parallelism.
%The process of the \substep{s} finish when some condition, noted as $\cstop$, is satisfied. In many cases, it $\cstop{}$ just determines if no new vertices are pulled into the frontier.

We argue that, this mechanism of allowing for the growth of the frontier, is the main feature that makes a priority queue ``batched'' instead of ``streaming'' (dealing with one element at a time), and ``parallel'' instead of ``serial'', in the \sssp{} problem.
In fact, most of the previous \sssp{} algorithms falls into this framework in Algorithm \ref{algo:sssp}. In Table \ref{tab:allsssp}, we list a few examples including the parallel Dijkstra's, parallel Bellman-Ford, \deltastepping{}, \radiusstepping{} and Shi and Spencer's algorithm. Their use of priority queue boils down to different choices of the two conditions: $\condex$, which is the condition to extract the frontier, and $\condadd$, which decides if a vertex should be added to the current frontier. We note that the pseudocode only presents the conceptual idea of these algorithms, which may not reflect the real implementation details.

In this project, by better understanding the semantics and designing an efficient implementation of the \sbpq{}, our goal is to achieve an efficient parallel \sssp{} algorithm. We will first need to understand the challenge in the parallel \sssp{} algorithm, which is the hardness of getting both span and work low (also known as the transitive-closure bottleneck). Intuitively, for a frontier-based algorithm, the tradeoff embodies in the choice of the frontier size. Choosing a large frontier means to select the vertices for relaxation more aggressively. More vertices can be processed in parallel, but likely much of the work is redundant. We say a vertex $v$ is settled if its tentative distance equals to the real shortest distance, and unsettled otherwise. If an unsettled vertex is used to relax its neighbors, then all work is \emph{ineffective}.
Having more vertices processed in parallel results in more unsettled vertices being processed.
An extreme case of large frontier is the parallel Bellman-Ford algorithm where the frontier is always all vertices. The algorithm will finish in $O(T_{\mathtext{sssp}})$ \step{s}, where $T_{\mathtext{sssp}}$ is the shortest path tree depth. We note that without shortcutting, this is the lower bound for the number of \step{s}. However the total work is $O(mn)$.
Especially when the graph is sparse and the shortest path tree is deep, this overhead is significant. For example, in most road networks with millions of vertices, the number of effective updates in each \step{} is usually only a few hundreds, and thus the extra work is unaffordable.
On the other hand, using a small frontier selects the vertices for relaxation more conservatively, which avoids ineffective work. However it increases the number of \step{s} needed. Once a vertex is settled, we want to process it as soon as possible, instead of waiting until it is on the top of the priority queue. An extreme case is the parallel Dijkstra's algorithm where the frontier is always just the closest vertex. While no redundant work is done, the algorithm suffers from $\Omega(n)$ span. This long dependence is more significant especially in dense graphs where the shortest path tree is shallow. In fact, in most social networks with billions of vertices, the parallel Bellman-Ford finishes in no more than 50 rounds. Therefore, only using a small frontier delays many effective updates, and harms parallelism.

We plan to tackle this problem, both in theory and in practice. By carefully inspecting and understanding previous algorithms, we propose several simple conditions $\condex$ and $\condadd$ for \sbpq{}. Some initial experiments show that our algorithm is efficient, and outperforms many existing algorithms (see details below). We plan to study the theory behind the practical results. If successful, we believe we can achieve the first practical parallel \sssp{} algorithm with non-trivial worst-case cost bounds.
In summary, our goals include the following.

\begin{itemize}
  \item Design the interface of a parallel \bpq{} and its implementation.
  \item Design a parallel \sssp{} that uses \bpq{}, that is practical and theoretically efficient (provable worst-case work and span bounds). We hope that our algorithm could avoid using structure-based parameter. If necessary, parameters could depend on the number of vertices and edges.
  \item Apply the \sssp{} algorithm to more algorithms. Currently we believe the same data structure applies to s-t shortest path, $A^*$ search, and possibly Huffman tree construction.
  \item For an original algorithm that uses priority queues, formalize the condition that a \bpq{} data structure could be used to parallelize the original problem. This includes both the correctness guarantee and possibly cost bounds.
\end{itemize}


\textbf{Preliminary Experimental results.} Based on the framework in Algorithm \ref{algo:sssp}, we designed two simple heuristics of the priority queue. The core idea is to keep the simplicity and practicability of the \deltastepping{} algorithm, while absorbing the merits in the theoretically-efficient algorithms.
The two strategies, noted as \ssspours{}-Dense and \ssspours{}-Sparse, are designed for dense and sparse graphs respectively.
The initial frontier size $\ssspth$ is a fixed size $\ssspth$ of the current queue.
As mentioned, in a dense version, the number of \step{s} is likely small. In this case we can afford processing many vertices in a \step{} to let the tentative distance drop quickly.
To avoid too much redundant work, we also assign closer vertices higher priorities to let them be processed in earlier \substep{s}.
Therefore in the current $Q$, we identify $d_j$ as the distance of the $j\cdot \ssspth$-th element smallest. These distance thresholds are used as virtual ``barriers'' to make use of the priority information to roughly order the vertices in the frontier.
In a sparse version, also as mentioned, the main goal is to reduce ineffective work, and thus we focus on first settling all vertices within distance $d_1$, which is some threshold based on the current frontier. We implemented these two simple strategies, each taking about 200 lines of code, to existing \sssp{} algorithms in highly-optimized graph processing systems, including Ligra \cite{}, Julienne \cite{}, GAPBS, and Galois. We use different graphs types, with up to billions of vertices and edges. Our light-weighted implementation outperforms xx in xxx and xx in xx. We believe our current version is highly practical. We also believe that by further studying the theory, our implementation could get even better performance.

\textbf{Theoretical Study Directions.} As mentioned, theoretically-efficient \sssp{} algorithm is hard, and reducing both work and depth of the problem is conjectured to be impossible. As mentioned, without adding shortcuts, the lower bound of span is the shortest distance tree depth. However adding shortcuts could be impractical because the number of needed shortcuts is usually much more than the input edges. We propose to study the parameterized bounds. This means that the bound is possibly tied to some properties of the input graph. One example is to bound the span in the shortest path tree depth of the graph. Another formalization we believe useful is the $(k,\rho)$-graph proposed by the PIs in 2016 \cite{}. Informally, a $(k,\rho)$-graph means that any vertex can reach its $\rho$-nearest neighbors in $k$-hops. This basically says that by $k$ \substep{s}, a settled vertex can settle another $\rho$ vertices. This concept has been used to show the theoretical results in \radiusstepping{} \cite{}. We believe it is the key factor that affects how much parallelism we can achieve in an \sssp{} algorithm. We would like to provide analysis and worst-case bound based on the concept of $(k,\rho)$-graph.
%In fact, both \radiusstepping{} \cite{} and Shi and Spencer's \cite{} requires to preprocess a graph to a $(1,\rho)$-graph by adding at most $n\rho$ shortcuts in $O(m\log n+n\rho^2)$ work and $O(\rho^2)$ span. For achieving a non-trivial bound, $\rho$ should be set to $n^{\epsilon}$ for $0<\epsilon<1$, which makes both the space and time cost large. We believe that using

\textbf{Generalization. } If successful, we believe our approach is applicable to other algorithms, including s-t shortest path, $A^*$, and Huffman tree construction. We plan to study the the condition that a \sbpq{} data structure could be used to parallelize the original problem using a regular \pq{}. This includes both the correctness guarantee and cost bounds.








\begin{algorithm}[t]
\caption{Parallel SSSP algorithm framework using soft priority queue}
\label{algo:sssp}
\SetKwProg{mystruct}{struct}{}{}
\SetKwProg{myfunc}{function}{}{}
\SetKwFor{ParForEach}{parallel foreach}{do}{endfch}
\KwIn{Weighted input graph $G(V, E)$, source $s$}
\KwOut{Shortest distance $d(\cdot)$ of all vertices to $s$}
%\KwMaintains{Parallel batch priority queue}
  \vspace{.5em}
Initialize $d(s)=0$, and all other $d(v)=\infty$ for $v\ne s$. Add $s$ to SoftPQ $\mathtext{\pq}$\\
\While(\tcp*[f]{\textbf{\step{s}}}) {$\mathtext{\pq}$ is not empty} {
  $\frontiersymbol\gets\mathtext{\pq}$.extract($\condex$) \tcp*{get the initial frontier}
  %$\frontiersymbol\gets \frontiersymbol_0$ \\
  %\While(\tcp*[f]{\textbf{\substep{s}}. $\cstop$ is some stop condition}) {$\neg \cstop$} {
  %  $\frontiersymbol \gets \pq$.relax\_and\_add($\frontiersymbol, \condadd$)\tcp*{process and get next sub-frontier}
  %}
  \lWhile(\tcp*[f]{\textbf{\substep{s}}}.) {$\frontiersymbol'\ne \emptyset$} {
    $\frontiersymbol \gets \pq$.relax\_and\_add($\frontiersymbol, \condadd$)%\tcp*{process and get next sub-frontier}
  }
}
\vspace{.5em}
\mystruct{$\text{SoftPQ}$}{
  Let $Q$ be the set of all elements in this soft priority queue\\
  \myfunc{$\frontiersymbol=$extract($\condex$)} {
    $\frontiersymbol \gets $All vertices in $Q$ with condition $\condex$\\
    Remove $\frontiersymbol$ from $Q$\\
  }
  \vspace{.2em}
  \myfunc{$\frontiersymbol'=$relax\_and\_add($\frontiersymbol, \condadd$)} {
    $\frontiersymbol' \gets \emptyset$\\
    \ParForEach {$v\in \frontiersymbol$} {
        \ParForEach{$u$ is neighbor of $v$} {
          \If {$v$ relaxes $u$} {
            \lIf {$\condadd(u)$} {Add $u$ to $\frontiersymbol'$. Remove $u$ from $Q$ if $u\in Q$}
            \lElse{add $u$ to $Q$ if $u\notin Q$}
          }
        }
    }
  }
}
\end{algorithm}

\hide{
\begin{table}
  \centering
  \small
  \begin{tabular}{llll}
    % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
    \bf Algorithm & $\boldsymbol{\condex(u)}$ & $\boldsymbol{\condadd(u)}$ & $\boldsymbol{C_{\mathtext{stop}}}$ \\
    \hline
    Dijkstra's & $d(u)=\min_{v\in Q}$ & \false & $\frontiersymbol\neq \emptyset$\\
    Bellman-Ford & \true & \false & $\frontiersymbol\neq \emptyset$\\
    \deltastepping{} \cite{} & $d(u)\le i\Delta$, $i$ is the current step&$d(u)\le i\Delta$, $i$ is the current round& $\frontiersymbol\neq \emptyset$\\
    \radiusstepping{} \cite{} & $d(u)\le r_i$, $r_i$ is the current radius&$d(u)\le r_i$, $r_i$ is the current radius& $\frontiersymbol\neq \emptyset$\\
    Shi and Spencer \cite{}&$d(u)$ is top $k$ in $Q$, where $k$ is a & $d(u)$ is top $k$ in $Q\cup \frontiersymbol'$, and $u$ is & within 4\\
    &fixed parameter&within 4 hops from initial frontier& \substep{s}\\
    \hline
    \ssspours{}-Dense& $d(u)$ is in the top $k$ in $Q$, where & $d(u)$ is among the top $j\times k$ in $Q$, &within $h$ \\
    &$k$ is a constant fraction of $|Q|$ & $j$ is the current \substep{} &\substep{s} \\
    \ssspours{}-Sparse& $d(u)$ is in the top $k$ in $Q$, where& Return \true{} if $d(u)\le d'$ and $u$ is &within $h$ \\
    &$k=c|Q|$ for constant $c$&  within $h$-hops from the initial&\substep{s} \\
    &Let $d'=\max_{u}d(u)$ for $u$ in $\frontiersymbol$ & frontier. Return \false{} otherwise.& \\
    \hline
  \end{tabular}
  \caption{a}\label{tab:allsssp}
\end{table}
}

\hide{
\begin{table}
  \centering
  \small
  \begin{tabular}{lll}
    % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
    \bf Algorithm & $\boldsymbol{\condex(u)}$ & $\boldsymbol{\condadd(u)}$ \\
    \hline
    Dijkstra's & $d(u)=\min_{v\in Q}$ & \false\\
    Bellman-Ford & \true & \false\\
    \deltastepping{} \cite{} & $d(u)\le i\Delta$, $i$ is the current step&$d(u)\le i\Delta$, $i$ is the current round\\
    \radiusstepping{} \cite{} & $d(u)\le r_i$, $r_i$ is the current radius&$d(u)\le r_i$, $r_i$ is the current radius\\
    Shi and Spencer \cite{}&$d(u)$ is top $\ssspth$ in $Q$, where $k$ is a & $d(u)$ is top $\ssspth$ in $Q\cup \frontiersymbol'$ and $j\le 4$, \\
    &fixed parameter&where $j$ is the current round of \substep{}\\
    \hline
    \ssspours{}-Dense& $d(u)$ is top $\ssspth_0$ in $Q$, where & $d(u)$ is top $j\times \ssspth_0$ in $Q$ and $j\le h$, \\
    &$\ssspth=\ssspratio|Q|$ for constant ratio $\ssspratio_D$ & where $j$ is the current round of \substep{}, \\
    &&and $h_D$ is a fixed parameter.\\
    \ssspours{}-Sparse& $d(u)$ is in the top $\ssspth_S$ in $Q$, where& Return \true{} if $d(u)\le d'$ and $j\le h_S$, where\\
    &$\ssspth_S=\ssspratio_S|Q|$ for constant ratio $\ssspratio_S$& $j$ is the current round of \substep{}, and $h_S$ is a \\
    &Let $d'=\max_{u}d(u)$ for $u$ in $\frontiersymbol$ &fixed parameter. Return \false{} otherwise. \\
    \hline
  \end{tabular}
  \caption{a}\label{tab:allsssp}
\end{table}}

\begin{table}
  \centering
  \small
  \begin{tabular}{lll}
    % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
    \bf Algorithm & $\boldsymbol{\condex(u)}$ & $\boldsymbol{\condadd(u)}$ \\
    \hline
    Dijkstra's & $d(u)=\min_{v\in Q}$ & \false\\
    Bellman-Ford & \true & \false\\
    \deltastepping{} \cite{} & $d(u)\le i\Delta$, $i$ is the current step&$d(u)\le i\Delta$, $i$ is the current round\\
    \radiusstepping{} \cite{} & $d(u)\le r_i$, $r_i$ is the current radius&$d(u)\le r_i$, $r_i$ is the current radius\\
    Shi and Spencer \cite{}&$d(u)$ is top $\ssspth$ in $Q$, where $\ssspth$ is a & $d(u)$ is top $\ssspth$ in $Q\cup \frontiersymbol'$ and $j\le 4$, \\
    &fixed parameter&where $j$ is the current round of \substep{}\\
    \hline
    \ssspours{}-Dense& $d(u)<d_1$, where $d_j$ is set to be the &
    $u\in \frontiersymbol_0$ and $d(u)<d_j$ and $j\le h$, where $j$ is\\
    &distance of the $(j\cdot \ssspth_D)$-th smallest  &
     the current round of \substep{}, $\frontiersymbol_0$ the initial \\
    &element in current $Q$. $\ssspth_D$ is a constant&
    frontier, and $h_D$ a fixed parameter.\\
    \ssspours{}-Sparse& $d(u)<d_1$, where $d_1$ is set to be the &
    Return \true{} if $d(u)\le d_1$ and $j\le h_S$, where\\
    &distance of the $\ssspth_S$-smallest element&
    $j$ is the current round of \substep{}, and $h_S$ a \\
    & in current $Q$. $\ssspth_S$ is a constant&
    fixed parameter. Return \false{} otherwise. \\
    \hline
  \end{tabular}
  \caption{a}\label{tab:allsssp}
\end{table}





==> connectivity.tex <==
\section{Parallel Batch-Dynamic Priority Queue}
\label{sec:sssp}
Another typical example of the abstract data type (ADT) is the priority queue (\pq{}).
A priority queue maintains a set of elements with keys as priorities, and supports three primitives: \mf{Extract-Min} that pops the element with the smallest key, \mf{Insert} that adds a new element, and \mf{Dec-Key} that decreases the key of an element.
Other operations such as \mf{Delete} or \mf{Update} can be implemented via these primitives.
Priority queues have many applications, such as in Prim's algorithm~\cite{prim1957shortest} for computing minimum spanning tree, constructing a Huffman tree~\cite{huffman1952method}, and best-first searches~\cite{pearl1984intelligent}.
The most famous application of priority queues is probably in Dijkstra's algorithm for single-source shortest paths (\sssp{}) on a graph.
Sequentially, Dijkstra's algorithm uses a priority queue and it is simple and practical.
Similar to the previous section, we will use SSSP and Dijkstra as a motivating example of parallel priority queues.

As opposed to many other graph algorithms, SSSP is notoriously hard in the parallel setting.
To date, there is no work-efficient solution with a non-trivial ($o(n)$) span bound, where $n$ is the number of vertices.
Directly parallelizing Dijkstra's leads to $\Omega(n)$ span due to the use of priority queue: \mf{Extract-Min} pops one vertex at a time for $n$ times in total.
Thus, it is natural to ask if we can parallelize the priority queue.

\myparagraph{Parallelizing priority queue.} There are two major approaches for parallelizing the priority queue.
One is to allow concurrent updates to the priority queue~\cite{alistarh2015spraylist,sundell2005fast,linden2013skiplist,shavit2000skiplist,liu2012lock,henzinger2013quantitative}, and the implementations are based on skip-lists.
The other is to relax the priority queue to allow batch updates and batch extracts on $k$ elements, so multiple processors can work on different vertices simultaneously.
To support these functions, the underlying data structure is a search tree~\cite{blelloch2016parallel}, which can be either the parallel search trees by the PI Sun and coauthors~\cite{Blelloch2016just,sun2018pam,sun2019parallel} in the shared-memory setting, or B-trees~\cite{bingmann2015bulk,sanders2019sequential} in the distributed and external-memory settings.
Unfortunately, maintaining either a skip-list or a search tree is very costly because the total ordering of all elements is kept, which is not required in the sequential heap implementations.

\myparagraph{Practical approaches for SSSP.} Due to the aforementioned problems, practical parallel SSSP algorithms \emph{do not} use the parallel priority queue abstraction.
In practice, Bellman-Ford~\cite{bellman1958routing,ford1956network} can easily be parallelized by relaxing all edges in one round simultaneously, and it performs very well on small-diameter graphs~\cite{ShunB2013,zhang2018graphit}.
Bellman-Ford does not use a priority queue.
Inspired by the good performance of Bellman-Ford, practical parallel SSSP implementations~\cite{zhang2020optimizing,dhulipala2017,nguyen2013lightweight,beamer2015gap} are based on $\Delta$-stepping~\cite{meyer2003delta}, which is a generalization of Bellman-Ford.
In practice, these implementations are faster than those using priority queues since they use flat arrays but not a tree-based priority queue.
However, given a graph with $n$ vertices and $m$ edges, $\Delta$-stepping requires $O(nm)$ work and $O(n)$ span in the worst case, which is no better than the simpler Bellman-Ford.
Also, the parameter $\Delta$ in $\Delta$-stepping highly depends on the input graph structure and the distribution of edge weights, and its best choice is not known without exhaustive searching on each input graph instance~\cite{zhang2020optimizing}.

\myparagraph{Theoretical approaches for SSSP.}
Given the importance of SSSP, there has been a rich literature of theoretical parallel algorithms~\cite{ullman1991high,klein1997randomized,cohen1997using,Shi1999,cohen2000polylog,spencer1997time,blelloch2016parallel} that uses $o(nm)$ work and $o(n)$ span.
Unfortunately, all of these algorithms have some issues that make them potentially impractical on real-world large-scale graphs, including the latest, conceptually simpler algorithm \radiusstepping{}~\cite{blelloch2016parallel} proposed by both PIs and coauthors in 2016 (see more details later).
All of these algorithms~\cite{blelloch2016parallel,Shi1999,ullman1991high,klein1997randomized,cohen1997using} relies on some assumptions which make them potentially impractical.
For instance, they all use shortcuts or hopsets to get the corresponding bounds.
To achieve $O(n^{1-\epsilon})$ span in these algorithms, we need to add $\Omega(m^{1+\epsilon})$ shortcut edges.
In practice, the memory size of a single machine can only store the edges in large real-world graphs, and cannot afford to store asymptotically more shortcut edges.
As a result, to date, the problem for exact parallel SSSP remains open:
\begin{center}
  \emph{Q2: Is there a parallel SSSP algorithm that is both practically efficient (faster than Bellman-Ford and $\Delta$-stepping in performance), and theoretically efficient (at least have better bounds than Bellman-Ford)?}
\end{center}

We propose to answer \emph{Q2} by combining existing theoretical and practical results.
On the theory side, the \radiusstepping{} paper~\cite{blelloch2016parallel} proposed a concept of $(k,\rho)$-graph, which we believe is useful to analyze parallel SSSP algorithms.
On the practical side, we would like to take implementation details into consideration, and in particular, to avoid using expensive shortcuts or hopsets, or tree-based data structure.

\myparagraph{Proposed work: Parallel Batch-Dynamic Priority Queue (\dbpq{})}.
We believe that \emph{Q2} is a long-standing open problem is due to the lack of a good abstract data type (ADT) of the parallel priority queue. A good abstraction of priority queue should be able to unify the three aspects as discussed above: theory research on parallel SSSP algorithm design and analysis, data structure research for parallel priority queue, and system/software research on parallel SSSP implementation.
Unfortunately, existing work on parallelizing priority queues~\cite{alistarh2015spraylist,sundell2005fast,linden2013skiplist,shavit2000skiplist,liu2012lock,henzinger2013quantitative,bingmann2015bulk,sanders2019sequential} are only used in Dijsktra, not to other theoretical or practical approaches;
existing theoretical approaches~\cite{ullman1991high,klein1997randomized,cohen1997using,Shi1999,cohen2000polylog,spencer1997time,blelloch2016parallel} do not explicitly use parallel priority queues and do not have experimental evaluations;
existing practical implementations~\cite{zhang2020optimizing,dhulipala2017,nguyen2013lightweight,beamer2015gap} are done by the software and system community and they only optimize $\Delta$-stepping, not other algorithms and data structures.
Given the difficulty of parallel SSSP, it seems less likely that a single solution can magically solve all challenges.
We hope our proposed work can help to combine and connect the three aspects in parallel SSSP research.
We believe defining the following abstraction will be very helpful.

\begin{definition}[Batch-PQ]
For a data structure $\mathq{}$ implementing the \dbpq{}, it stores a set of keys for elements in $S$, and supports the following three operations:

\begin{itemize}[topsep=1.5pt, partopsep=0pt,itemsep=0pt]
  \item $\mf{Extract}(\cond)$: extract the set of $s\in S$ such that $\cond(s)$ is true for a user-defined predicator $\cond$,
  \item $\mf{B-Insert}(S')$: batch insertion, which updates $\mathq$ to contain $S\cup S'$,
  \item $\mf{B-Update}(S', \rel{})$: batch update, which updates the keys of elements in $S'$ using function \rel{}.
\end{itemize}
\end{definition}

At first glance, it may seem that the \dbpq{} interface is similar to the previous parallel priority queue~\cite{bingmann2015bulk,sanders2019sequential}, which can extract or update a batch of $k$ elements instead of one element.
However, we note that the main difference is that we allow a user-specific predicator $\cond$ to extract the elements, which supports a much stronger functionality.
For instance, \dbpq{} can be used to implement parallel Bellman-Ford with $\cond(v)\equiv \True$ and to relax their neighbor vertices using $\mf{B-Insert}$ and $\mf{B-Update}$, but it seems hard with the interface of the previous parallel priority queue (e.g., $k\mf{-Extract}$ and $k\mf{-Update}$).
Although we omit the details of previous algorithms due to space limitations, we note that the interface for \dbpq{} can easily be used to implement practical SSSP algorithms such as $\Delta$-stepping, and theoretical SSSP algorithms such as \radiusstepping{}~\cite{blelloch2016parallel} and Shi and Spencer's~\cite{Shi1999}, albeit requiring light modifications.
%\footnote{It requires some simplifications of these algorithms, so in the preliminary experiment we rename the simplified version of \radiusstepping{} as \newalgo{} to avoid confusions.}v

Therefore, with the \dbpq{} interface, all three previously isolated areas are connected.
The implementation tricks such as the smart use of flat arrays in~\cite{zhang2020optimizing,dhulipala2017,nguyen2013lightweight,beamer2015gap} can inspire the implementation for theoretical algorithms since they share the same underlying implementation for \dbpq{}.
The theoretical analysis in~\cite{blelloch2016parallel,Shi1999} still holds once we plug in the cost bounds for the \dbpq{} operations.
Also, when we design or implement parallel SSSP algorithms, we can treat the \dbpq{} as a black box, which greatly simplifies the thought process; however, that was not the case when designing previous algorithms either theoretically~\cite{ullman1991high,klein1997randomized,cohen1997using,Shi1999,cohen2000polylog,spencer1997time,blelloch2016parallel} or practically~\cite{zhang2020optimizing,dhulipala2017,nguyen2013lightweight,beamer2015gap}.
We believe the \dbpq{} interface bridges together the theoretical algorithms and analysis, data structure design, and implementation details.
Therefore, we are optimistic about answering \emph{Q2} and designing parallel SSSP algorithms that are efficient both theoretically and practically.


\textbf{Theoretical Study Directions.}
Aiming at bridging the gap between theory and practice, we combined some theory insights in \radiusstepping{} and some ideas in practical implementations of \deltastepping{}~\cite{zhang2020optimizing,dhulipala2017}, as well as the \dbpq{} abstraction as proposed above. Bringing them together, we designed a preliminary parallel SSSP algorithm \ssspours{}.
The reason we pick \radiusstepping and \deltastepping is that they all run in steps, and in each step, the algorithms ``settle down'' the SSSP distances for vertices in a ``range''.
The difference between \radiusstepping and \deltastepping is that, \deltastepping uses a fixed range, while \radiusstepping computes a distance range in each step that provides efficient cost bounds.
\ssspours{} adopts the idea similar to \radiusstepping that dynamically decides the distance range, and the implementation of \dbpq{} is a flat array-structure similar to \deltastepping.
Such implementation avoids using the tree-base structure and does not add shortcut edges.
As such, \ssspours{} is already very efficient in practice (Figure~\ref{fig:prelim}(b)), but again does not have interesting bounds.

The first question we would like to study is an efficient design for \dbpq.
Our goal is to achieve better bounds than using the flat array in \deltastepping, and the search-tree in \radiusstepping that is not work-efficient and practically inefficient due to the pointer-based structure.
Our goal is a hierarchical structure that provides improved bounds, and can be implemented based on arrays that is fast in practice.

The second question is about the bounds for the SSSP algorithm.
Since we cannot add shortcuts in practice, showing interesting worst-case bounds seems much more challenging---there is no much we can do for a chain without adding shortcuts.
However, we believe we can achieve parameterized bounds.
This means that the bounds are possibly tied to some properties of the input graph.
We believe that the concept of $(k,\rho)$-graph proposed by the PIs in 2016~\cite{blelloch2016parallel} can be helpful.
Informally, a $(k,\rho)$-graph means that any vertex can reach its $\rho$-nearest neighbors in $k$-hops.
This basically means that by $k$ \substep{s}, a settled vertex can further settle $\rho$ vertices.
This concept was used to prove the bounds of \radiusstepping{}, and seems to be the key factor on how much parallelism we can achieve in \sssp{}.
Hence, the PIs propose to explore what parameterized bounds we can show for practical SSSP algorithms, with the tools of \dbpq and $(k,\rho)$-graph.
It seems that showing the bounds for \ssspours is promising due to the similarity to \radiusstepping.

%In fact, both \radiusstepping{} \cite{} and Shi and Spencer's \cite{} requires to preprocess a graph to a $(1,\rho)$-graph by adding at most $n\rho$ shortcuts in $O(m\log n+n\rho^2)$ work and $O(\rho^2)$ span. For achieving a non-trivial bound, $\rho$ should be set to $n^{\epsilon}$ for $0<\epsilon<1$, which makes both the space and time cost large. We believe that using

\textbf{Preliminary Experimental Results.}
As a proof-of-concept, we implemented \ssspours{} and compared it to state-of-the-art SSSP implementations (see Figure~\ref{fig:prelim}(b)).
%The computation of the range can be done via the $\cond$ function, and we implemented an initial version (\ssspours) with the running time shown in Figure~\ref{fig:prelim}(b).
We can see that even our preliminary version is already faster than the state-of-the-art graph processing systems on almost all graphs.
This indicates the practicability of our solution.
We will keep exploring better implementations, especially by exploring the parameter space of \ssspours, which seems promising using the \dbpq{} abstraction.
We will also improve the algorithm according to the progress on the theoretical side of the algorithm.
%We also plan to implement existing algorithms such as Bellman-Ford and \deltastepping based on \dbpq{}, and to compare them to the existing software.
% given the \dbpq as our secret weapon.

\myparagraph{Other applications using \dbpq{}.}
We note that many problems with sequential algorithms using priority queues remain unsolved in the parallel setting.
We believe the reason is the lack of an elegant interface of the parallel priority queue and efficient underlying implementation.
If the previously proposed work is successful, we can consider \dbpq as a black box and apply it to many other algorithms.

One possible topic to study is other shortest-paths problems such as $s$-$t$ shortest path and $A^*$ search.
There are many textbook algorithms to solve these problems sequentially~\cite{CLRS} by using priority queues.
If the design of \dbpq{} is successful, we want to explore whether we can solve these problems in parallel.

Another interesting question to explore is when the parallel priority queue can be used.
For instance, we cannot directly use \dbpq{} to parallelize Prim's algorithm since we can only guarantee the smallest edge in the priority queue is in the MST, and not even for the second smallest.
The reason we can use \dbpq{} in SSSP is that SSSP allows ``priority-inversion''~\cite{alistarh2019efficiency}.
However, we believe this property is too strong.
In fact, we believe \dbpq{} can be used in more applications such as constructing Huffman tree, which is another typical use case of priority queue but does not allow priority-inversion.
We plan to study the theoretical question about the accurate boundary when \dbpq{} can apply correctly. 
